Automated Controller Calibration by Kalman Filtering

This paper proposes a method for calibrating control parameters. Examples of such control parameters are gains of PID controllers, weights of a cost function for optimal control, filter coefficients, the sliding surface of a sliding mode controller, or weights of a neural network. Hence, the proposed method can be applied to a wide range of controllers. The method uses a Kalman filter that estimates control parameters, using data of closed-loop system operation. The control parameter calibration is driven by a training objective, which encompasses specifications on the performance of the dynamical system. The performance-driven calibration method tunes the parameters online and robustly, is computationally efficient, has low data storage requirements, and is easy to implement making it appealing for many real-time applications. Simulation results show that the method is able to learn control parameters quickly, is able to tune the parameters to compensate for disturbances, and is robust to noise. A simulation study with the high-fidelity vehicle simulator CarSim shows that the method can calibrate controllers of a complex dynamical system online, which indicates its applicability to a real-world system. We also verify the real-time feasibility on an embedded platform with automotive-grade processors by implementing our method on a dSPACE MicroAutoBox-II rapid prototyping unit.

==> 2023TCST_accepted - Kalman Controller Calibration/fig/blockdiagram.tex <==
    %\includegraphics{}
    % Define block styles
    \tikzstyle{decision} = [diamond, draw, fill=blue!20, text width=4.5em, text badly centered, node distance=6cm, inner sep=0pt]
    \tikzstyle{block} = [rectangle, draw, fill=white!20, text width=5em, text centered, rounded corners, minimum height=4em, node distance=3cm]
    \tikzstyle{line} = [draw, -latex']
    \tikzstyle{cloud} = [draw, ellipse,fill=red!20, node distance=3cm, minimum height=2em]
    
    \begin{tikzpicture}[node distance = 2cm, auto]
    \node [block,text width=8em] (tuning) {Kalman Filter Calibration Module};
    \node [block]at(3,0) (safe) {Safety Check};
    \path [line] (safe) --  (4,-3);
    \node [block]at(3.5,-2) (mpc) {Controller};
    \node [block]at(6,-2) (plant) {Dynamical System};
    %\node [below of=plant] (line1) {};
    % Place nodes
    \node []at(3.5,-1) {$\theta$};
    \path [line] (tuning) -- (safe);
    \path [line] (mpc) -- (plant);
    \path [line] (plant) -- (6,-3.25) -- (0,-3.25) -- (tuning);
    \path [line] (plant) -- (6,-3.25) -- (0,-3.25) -- (0,-2) -- (mpc);
    \end{tikzpicture} 

